Explainable AI in 6G O-RAN: A Tutorial and Survey on Architecture, Use Cases, Challenges, and Future Research

The recent O-RAN specifications promote the evolution of RAN architecture by function disaggregation, adoption of open interfaces, and instantiation of a hierarchical closed-loop control architecture managed by RAN Intelligent Controllers (RICs) entities. This paves the road to novel data-driven network management approaches based on programmable logic. Aided by Artificial Intelligence (AI) and Machine Learning (ML), novel solutions targeting traditionally unsolved RAN management issues can be devised. Nevertheless, the adoption of such smart and autonomous systems is limited by the current inability of human operators to understand the decision process of such AI/ML solutions, affecting their trust in such novel tools. eXplainable AI (XAI) aims at solving this issue, enabling human users to better understand and effectively manage the emerging generation of artificially intelligent schemes, reducing the human-to-machine barrier. In this survey, we provide a summary of the XAI methods and metrics before studying their deployment over the O-RAN Alliance RAN architecture along with its main building blocks. We then present various use cases and discuss the automation of XAI pipelines for O-RAN as well as the underlying security aspects. We also review some projects/standards that tackle this area. Finally, we identify different challenges and research directions that may arise from the heavy adoption of AI/ML decision entities in this context, focusing on how XAI can help to interpret, understand, and improve trust in O-RAN operational networks.

==> acro_table.tex <==
\begin{table*}[t!]
\caption{List of Acronyms}
\label{tab:acro}
\centering 
\begin{tabular}{|l|l||l|l|}
\hline
\textbf{\acrshort{3gpp}}		&	\acrlong{3gpp}			&	\textbf{\acrshort{non rt ric}}	&	\acrlong{non rt ric}	\\ \hline
\textbf{\acrshort{4g}}			&	\acrlong{4g}			&	\textbf{\acrshort{nr-mac}}		&	\acrlong{nr-mac}		\\ \hline
\textbf{\acrshort{5g}}			&	\acrlong{5g}			&	\textbf{\acrshort{ns}}			&	\acrlong{ns}			\\ \hline
\textbf{\acrshort{6g}}			&	\acrlong{6g}			&	\textbf{\acrshort{o-cloud}}		&	\acrlong{o-cloud}		\\ \hline
\textbf{\acrshort{a2c}}			&	\acrlong{a2c}			&	\textbf{\acrshort{o-cu-cp}}		&	\acrlong{o-cu-cp}		\\ \hline
\textbf{\acrshort{ai}}			&	\acrlong{ai}			&	\textbf{\acrshort{o-cu-up}}		&	\acrlong{o-cu-up}		\\ \hline
\textbf{\acrshort{ann}}			&	\acrlong{ann}			&	\textbf{\acrshort{o-cu}}		&	\acrlong{o-cu}			\\ \hline
\textbf{\acrshort{api}}			&	\acrlong{api}			&	\textbf{\acrshort{o-du}}		&	\acrlong{o-du}			\\ \hline
\textbf{\acrshort{b5g}}			&	\acrlong{b5g}			&	\textbf{\acrshort{o-ran}}		&	\acrlong{o-ran}			\\ \hline
\textbf{\acrshort{bbu}}			&	\acrlong{bbu}			&	\textbf{\acrshort{o-ru}}		&	\acrlong{o-ru}			\\ \hline
\textbf{\acrshort{bs}}			&	\acrlong{bs}			&	\textbf{\acrshort{opex}}		&	\acrlong{opex}			\\ \hline
\textbf{\acrshort{capex}}		&	\acrlong{capex}			&	\textbf{\acrshort{osc}}			&	\acrlong{osc}			\\ \hline
\textbf{\acrshort{cicd}}		&	\acrlong{cicd}			&	\textbf{\acrshort{pca}}			&	\acrlong{pca}			\\ \hline
\textbf{\acrshort{cnn}}			&	\acrlong{cnn}			&	\textbf{\acrshort{pdcch}}		&	\acrlong{pdcch}			\\ \hline
\textbf{\acrshort{cp}}			&	\acrlong{cp}			&	\textbf{\acrshort{pdcp}}		&	\acrlong{pdcp}			\\ \hline
\textbf{\acrshort{ct}}			&	\acrlong{ct}			&	\textbf{\acrshort{pdsch}}		&	\acrlong{pdsch}			\\ \hline
\textbf{\acrshort{cu}}			&	\acrlong{cu}			&	\textbf{\acrshort{phy}}			&	\acrlong{phy}			\\ \hline
\textbf{\acrshort{dag}}			&	\acrlong{dag}			&	\textbf{\acrshort{pnf}}			&	\acrlong{pnf}			\\ \hline
\textbf{\acrshort{darpa}}		&	\acrlong{darpa}			&	\textbf{\acrshort{pucch}}		&	\acrlong{pucch}			\\ \hline
\textbf{\acrshort{devops}}		&	\acrlong{devops}		&	\textbf{\acrshort{pusch}}		&	\acrlong{pusch}			\\ \hline
\textbf{\acrshort{dlift}}		&	\acrlong{dlift}			&	\textbf{\acrshort{qoe}}			&	\acrlong{qoe}			\\ \hline
\textbf{\acrshort{dl}}			&	\acrlong{dl}			&	\textbf{\acrshort{qos}}			&	\acrlong{qos}			\\ \hline
\textbf{\acrshort{dnn}}			&	\acrlong{dnn}			&	\textbf{\acrshort{r2}}			&	\acrlong{r2}			\\ \hline
\textbf{\acrshort{dqn}}			&	\acrlong{dqn}			&	\textbf{\acrshort{ran}}			&	\acrlong{ran}			\\ \hline
\textbf{\acrshort{drl}}			&	\acrlong{drl}			&	\textbf{\acrshort{rapp}}		&	\acrlong{rapp}			\\ \hline
\textbf{\acrshort{du}}			&	\acrlong{du}			&	\textbf{\acrshort{rat}}			&	\acrlong{rat}			\\ \hline
\textbf{\acrshort{embb}}		&	\acrlong{embb}			&	\textbf{\acrshort{reco}}		&	\acrlong{reco}			\\ \hline
\textbf{\acrshort{enb}}			&	\acrlong{enb}			&	\textbf{\acrshort{ric}}			&	\acrlong{ric}			\\ \hline
\textbf{\acrshort{eni}}			&	\acrlong{eni}			&	\textbf{\acrshort{rl}}			&	\acrlong{rl}			\\ \hline
\textbf{\acrshort{etsi}}		&	\acrlong{etsi}			&	\textbf{\acrshort{rm}}			&	\acrlong{rm}			\\ \hline
\textbf{\acrshort{fl}}			&	\acrlong{fl}			&	\textbf{\acrshort{rnn}}			&	\acrlong{rnn}			\\ \hline
\textbf{\acrshort{gan}}			&	\acrlong{gan}			&	\textbf{\acrshort{rss}}			&	\acrlong{rss}			\\ \hline
\textbf{\acrshort{gnb}}			&	\acrlong{gnb}			&	\textbf{\acrshort{rt}}			&	\acrlong{rt}			\\ \hline
\textbf{\acrshort{gnn}}			&	\acrlong{gnn}			&	\textbf{\acrshort{ru}}			&	\acrlong{ru}			\\ \hline
\textbf{\acrshort{he}}			&	\acrlong{he}			&	\textbf{\acrshort{scm}}			&	\acrlong{scm}			\\ \hline
\textbf{\acrshort{ieee}}		&	\acrlong{ieee}			&	\textbf{\acrshort{sdn}}			&	\acrlong{sdn}			\\ \hline
\textbf{\acrshort{ig}}			&	\acrlong{ig}			&	\textbf{\acrshort{shap}}		&	\acrlong{shap}			\\ \hline
\textbf{\acrshort{iot}}			&	\acrlong{iot}			&	\textbf{\acrshort{sla}}			&	\acrlong{sla}			\\ \hline
\textbf{\acrshort{isg}}			&	\acrlong{isg}			&	\textbf{\acrshort{smo}}			&	\acrlong{smo}			\\ \hline
\textbf{\acrshort{kl}}			&	\acrlong{kl}			&	\textbf{\acrshort{sm}}			&	\acrlong{sm}			\\ \hline
\textbf{\acrshort{lime}}		&	\acrlong{lime}			&	\textbf{\acrshort{svm}}			&	\acrlong{svm}			\\ \hline
\textbf{\acrshort{lo}}			&	\acrlong{lo}			&	\textbf{\acrshort{tti}}			&	\acrlong{tti}			\\ \hline
\textbf{\acrshort{lstm}}		&	\acrlong{lstm}			&	\textbf{\acrshort{ue}}			&	\acrlong{ue}			\\ \hline
\textbf{\acrshort{mac}}			&	\acrlong{mac}			&	\textbf{\acrshort{up}}			&	\acrlong{up}			\\ \hline
\textbf{\acrshort{mdp}}			&	\acrlong{mdp}			&	\textbf{\acrshort{urllc}}		&	\acrlong{urllc}			\\ \hline
\textbf{\acrshort{mec}}			&	\acrlong{mec}			&	\textbf{\acrshort{vbbu}}		&	\acrlong{vbbu}			\\ \hline
\textbf{\acrshort{mlops}}		&	\acrlong{mlops}			&	\textbf{\acrshort{vnf}}			&	\acrlong{vnf}			\\ \hline
\textbf{\acrshort{ml}}			&	\acrlong{ml}			&	\textbf{\acrshort{vo-cu}}		&	\acrlong{vo-cu}			\\ \hline
\textbf{\acrshort{mmtc}}		&	\acrlong{mmtc}			&	\textbf{\acrshort{vo-du}}		&	\acrlong{vo-du}			\\ \hline
\textbf{\acrshort{mm}}			&	\acrlong{mm}			&	\textbf{\acrshort{vran}}		&	\acrlong{vran}			\\ \hline
\textbf{\acrshort{mno}}			&	\acrlong{mno}			&	\textbf{\acrshort{wg}}			&	\acrlong{wg}			\\ \hline
\textbf{\acrshort{mvno}}		&	\acrlong{mvno}			&	\textbf{\acrshort{xai}}			&	\acrlong{xai}			\\ \hline
\textbf{\acrshort{near rt ric}}	&	\acrlong{near rt ric}	&	\textbf{\acrshort{xapp}}		&	\acrlong{xapp}			\\ \hline
\textbf{\acrshort{nfv}}			&	\acrlong{nfv}			&	\textbf{\acrshort{xr}}			&	\acrlong{xr}			\\ \hline
\textbf{\acrshort{ng ran}}		&	\acrlong{ng ran}		&				&				\\ \hline

\end{tabular}
\end{table*}


==> acro_table_backup <==
\begin{table*}[t!]
\caption{List of Acronyms}
\label{tab:acro}
\centering 
\begin{tabular}{|l|l||l|l|}
\hline
\textbf{Acronym}               & \textbf{Definition}&\textbf{Acronym}               & \textbf{Definition} \\ \hline \hline
\textbf{3GPP}                  & 3rd Generation Partnership Project&\textbf{NR-MAC}                & New Radio Medium Access Control  \\ \hline
\textbf{5G}                    & Fifth Generation&\textbf{NS}                    & Network Slicing   \\ \hline
\textbf{6G}                    & Sixth Generation &\textbf{O-CU}                  & Open RAN Central Unit \\ \hline
\textbf{A2C}                   & Advantage Actor Critic &\textbf{O-CU-CP}               & Open RAN Central Unit Control Plane \\ \hline
\textbf{AI}                    & Artificial Intelligence & \textbf{O-CU-UP}               & Open RAN Central Unit User Plane \\ \hline
\textbf{ANN}                   & Artificial Neutral Networks & \textbf{O-DU}                  & Open RAN Distributed Unit\\ \hline
\textbf{B5G}                   & Beyond Fifth-Generation & \textbf{O-RAN}                 & Open Radio Access Network\\ \hline
\textbf{BBU}                   & Baseband Unit &\textbf{O-RU}                  & Open RAN Radio Unit\\ \hline
\textbf{BS}                    & Base Station &\textbf{OPEX}                  & OPerational EXpenditures\\ \hline
\textbf{CAPEX}                 & CAPital EXpenditures &\textbf{OSC}                   & Open RAN Software Community\\ \hline
\textbf{CD/CI}                 & Continuous Delivery/Continuous Integration &\textbf{PCA}                   & Principal Component Analysis\\ \hline
\textbf{CNN}                   & Convolutional Neural Network &\textbf{PDCCH}                 & Physical Downlink Control Channel\\ \hline 
\textbf{CT}                    & Continuous Training &\textbf{PDCP}                  & Packet Data Control Protocol\\ \hline
\textbf{DARPA}                 & Defense Advanced Research Projects Agency & \textbf{PDSCH}  & Physical Downlink Shared Channel\\ \hline
\textbf{DevOps}                & DEVelopment and IT Operations & \textbf{PNF}                   & Physical Network Function\\ \hline
\textbf{DL}                    & Deep Learning &\textbf{PUCCH}                 & Physical Uplink Control Channel\\ \hline
\textbf{DNN}                   & Deep Neural Network &\textbf{PUSCH}                 & Physical Uplink Shared Channel\\ \hline
\textbf{DQN}                   & Deep Q-Network &\textbf{QoE}                   & Quality of Experience\\ \hline
\textbf{DRL}                   & Deep Reinforcement Learning &\textbf{QoS}                   & Quality of Service\\ \hline
\textbf{eMBB}                  & enhanced Mobile Broadband  &\textbf{RAN}                   & Radio Access Network\\ \hline
\textbf{ENI}                   & Experiential Networked Intelligence  &\textbf{RAT}                   & Radio Access Technologies\\ \hline 
\textbf{ETSI}                  & European Telecommunications Standards Institute &\textbf{RIC}                   & RAN Intelligent Controller\\ \hline
\textbf{FL}                    & Federated Learning &\textbf{RL}                    & Reinforcement Learning\\ \hline
\textbf{GAN}                   & Generative Adversarial Network  &\textbf{RNN}                   & Recurrent Neural Network\\ \hline
\textbf{gNB}                   & gNodeB  &\textbf{RT}                    & Real Time\\ \hline
\textbf{HE}                    & Horizon Europe &\textbf{SCM}                   & Structural Causal Models\\ \hline
\textbf{IEEE}                  & Institute of Electrical and Electronics Engineers &\textbf{SDN}                   & Software Defined Network\\ \hline
\textbf{IoT}                   & Internet of Things &\textbf{SHAP}                  & SHapley Additive exPlanations\\ \hline
\textbf{LIME}                  & Local Interpretable Model-Agnostic Explanations &\textbf{SLA}                   & Service Level Agreement\\ \hline
\textbf{LSTM}                  & Long Short Term Memory &\textbf{SM}                    & Spectrum Management\\ \hline
\textbf{MAC}                   & Medium Access Control &\textbf{SMO}                   & Service Management and Orchestration\\ \hline
\textbf{MDP}                   & Markov Decision Process &\textbf{SVM}                   & Support Vector Machines\\ \hline
\textbf{MEC}                   & Multi-access Edge Computing  &\textbf{TTI}                   & Transmission Time Interval\\ \hline
 \textbf{ML}                   & Machine Learning &\textbf{UE}                    & User Equipment\\ \hline
\textbf{MLOps}                 & ML system operations &\textbf{vBBU}                  & Virtual BBU\\ \hline
\textbf{mMTC}                  & massive Machine Type Communications &\textbf{VNF}                   & Virtual Network Function\\ \hline
\textbf{Near-RT RIC}           & Near Real-Time RAN Intelligent Controller &\textbf{vRAN}                  & Virtual RAN\\ \hline
\textbf{NFV}                   & Network Function Virtualization &\textbf{WG}                    & Working Group\\ \hline
\textbf{NG RAN}                & New Generation RAN &\textbf{\gls{xai}}                   & eXplainable AI\\ \hline
\textbf{Non-RT RIC}            & Non Real-Time RAN Intelligent Controller &\textbf{XR}                    & eXtended Reality\\ \hline

\end{tabular}
\end{table*}


==> acronyms_counter_zero_set.tex <==

\glsunset{3gpp}
\glsunset{4g}
\glsunset{5g}
\glsunset{6g}
\glsunset{a2c}
\glsunset{ai}
\glsunset{ann}
\glsunset{api}
\glsunset{b5g}
\glsunset{bbu}
\glsunset{bs}
\glsunset{capex}
\glsunset{cicd}
\glsunset{cnn}
\glsunset{cp}
\glsunset{ct}
\glsunset{cu}
\glsunset{dag}
\glsunset{dapp}
\glsunset{darpa}
\glsunset{devops}
\glsunset{dlift}
\glsunset{dl}
\glsunset{dnn}
\glsunset{dqn}
\glsunset{drl}
\glsunset{du}
\glsunset{embb}
\glsunset{enb}
\glsunset{eni}
\glsunset{etsi}
\glsunset{fl}
\glsunset{gan}
\glsunset{gnb}
\glsunset{gnn}
\glsunset{he}
\glsunset{ieee}
\glsunset{ig}
\glsunset{iot}
\glsunset{isg}
\glsunset{kl}
\glsunset{lime}
\glsunset{llm}
\glsunset{lo}
\glsunset{lstm}
\glsunset{mac}
\glsunset{mdp}
\glsunset{mec}
\glsunset{mlops}
\glsunset{ml}
\glsunset{mmtc}
\glsunset{mm}
\glsunset{mno}
\glsunset{mr}
\glsunset{mvno}
\glsunset{near rt ric}
\glsunset{nesy}
\glsunset{nfv}
\glsunset{ng ran}
\glsunset{non rt ric}
\glsunset{nr-mac}
\glsunset{ns}
\glsunset{o-cloud}
\glsunset{o-cu-cp}
\glsunset{o-cu-up}
\glsunset{o-cu}
\glsunset{o-du}
\glsunset{o-ran}
\glsunset{o-ru}
\glsunset{opex}
\glsunset{osc}
\glsunset{pca}
\glsunset{pdcch}
\glsunset{pdcp}
\glsunset{pdsch}
\glsunset{phy}
\glsunset{pnf}
\glsunset{pucch}
\glsunset{pusch}
\glsunset{qoe}
\glsunset{qos}
\glsunset{r2}
\glsunset{ran}
\glsunset{rapp}
\glsunset{rat}
\glsunset{reco}
\glsunset{ric}
\glsunset{rl}
\glsunset{rm}
\glsunset{rnn}
\glsunset{rss}
\glsunset{rt}
\glsunset{ru}
\glsunset{scm}
\glsunset{sdn}
\glsunset{shap}
\glsunset{sla}
\glsunset{smo}
\glsunset{sm}
\glsunset{svm}
\glsunset{tti}
\glsunset{ue}
\glsunset{up}
\glsunset{urllc}
\glsunset{vbbu}
\glsunset{vnf}
\glsunset{vo-cu}
\glsunset{vo-du}
\glsunset{vran}
\glsunset{wg}
\glsunset{xai}
\glsunset{xapp}
\glsunset{xr}

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
